Fast Batch Nuclear-norm Maximization and Minimization for Robust Domain Adaptation

Due to the domain discrepancy in visual domain adaptation, the performance of source model degrades when bumping into the high data density near decision boundary in target domain. A common solution is to minimize the Shannon Entropy to push the decision boundary away from the high density area. However, entropy minimization also leads to severe reduction of prediction diversity, and unfortunately brings harm to the domain adaptation. In this paper, we investigate the prediction discriminability and diversity by studying the structure of the classification output matrix of a randomly selected data batch. We find by theoretical analysis that the prediction discriminability and diversity could be separately measured by the Frobenius-norm and rank of the batch output matrix. The nuclear-norm is an upperbound of the former, and a convex approximation of the latter. Accordingly, we propose Batch Nuclear-norm Maximization and Minimization, which performs nuclear-norm maximization on the target output matrix to enhance the target prediction ability, and nuclear-norm minimization on the source batch output matrix to increase applicability of the source domain knowledge. We further approximate the nuclear-norm by L_{1,2}-norm, and design multi-batch optimization for stable solution on large number of categories. The fast approximation method achieves O(n^2) computational complexity and better convergence property. Experiments show that our method could boost the adaptation accuracy and robustness under three typical domain adaptation scenarios. The code is available at https://github.com/cuishuhao/BNM.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> abstract.tex <==
\IEEEtitleabstractindextext{%
	\begin{abstract}
		   
	\end{abstract}
	
	% Note that keywords are not normally used for peerreview papers.
	\begin{IEEEkeywords}
	Active learning, adversarial learning, self-supervised Learning, graph neural network.
\end{IEEEkeywords}}

==> document.tex <==
$\hat{\pi}=\underset{\pi \in \Pi_{G}^{N}}{\arg \max } \sum_{i}^{G} Q_{i, \pi(i)},$
where $Q_{i, \pi(i)}=\underbrace{\mathbb{1}\left[\pi(i) \in \Omega_{i}\right]}_{\text {spatial prior }} \cdot \underbrace{\left(\hat{p}_{\pi(i)}\left(c_{i}\right)\right)^{1-\alpha}}_{\text {classification }}$
$\underbrace{\left(\operatorname{IoU}\left(b_{i}, \hat{b}_{\pi(i)}\right)\right)^{\alpha}}_{\text {regression }} .$



\begin{table}[t]
	\begin{center}
		%\vspace{-5pt}
		
		\caption{Statistics on numbers of category samples for different datasets.}
		\vspace{-8pt}
		\label{samplenum}
		%\addtolength{\tabcolsep}{-5.5pt}
		\setlength{\tabcolsep}{1.3mm}{
			%\resizebox{\textwidth}{!}{%
			\begin{tabular}{ccccccc}
				%\multicolumn{2}{c}{R$\rightarrow$C}
				\hline
				Dataset & Domain & Sum  & Mean & Std &Max &Min  \\
				\hline\hline
				\multirow{2}*{Office-31}  &Amazon &2817 	&90.9 	&13.5 	&100 	&36\\ 
				&Dslr &498 	&16.1 	&5.7 	&31 	&7 \\
				\hline
				\multirow{2}*{Office-Home}  &Art &2427 	&37.3 	&19.6 	&99 	&15	\\ 
				&Clipart &4365 	&67.2 &24.1 &99 &39	 \\
				\hline
				\multirow{4}*{Domainnet}  &Clipart (train) &34019&98.6 &55.3 &328 &8	\\ 
				&Clipart (test) &14814&42.9&	23.7 &141&4		 \\
				&Real (train)&122563	&355.3 	&121.0 	&570 &21 \\
				&Real (test) & 52764	&152.9 	&51.8 &245 &10	 \\
				\hline
				\multirow{2}*{\shortstack{Semi\\Domainnet}}  &Clipart &18703	&148.4 	&87.9 	&469	&12\\ 
				&Real &70358	&558.4 	&142.4 	&804	&147\\
				\hline
				\multirow{4}*{\shortstack{Balanced\\Domainnet}}  &Clipart (train) &6300&50 &0 &50 &50\\ 				
				&Clipart (test) &2772&22&	0 &22&22	 \\
				&Real (train)&8568	&68 	&0 	&68 &68 \\
				&Real (test) & 3780	&30 	&0 &30 &30	 \\
				\hline
		\end{tabular}}%}
		\vspace{-10pt}
	\end{center}
\end{table}

==> experiment2.tex <==
\section{Experiments}
We apply our method to three domain adaptation situations, {\it i.e.}, unsupervised domain adaptation (UDA), semi-supervised domain adaptation (SSDA), and unsupervised open domain recognition (UODR). The experiments of the three tasks are accomplished on datasets of Office-31 \cite{saenko2010adapting}, Office-Home \cite{venkateswara2017deep}, Balance Domainnet, semi Domainnet~\cite{saito2019semi} and I2AwA~\cite{zhuo2019unsupervised}. We denote the direct entropy minimization and batch Frobenius-norm maximization as EntMin and BFM in our experiments. When BNMax and other methods cooperate with existing methods, we concatenate their names with ``+".

\subsection{Unsupervised Domain Adaptation}

Office-31 \cite{saenko2010adapting} and Office-Home \cite{venkateswara2017deep} are standard benchmarks for unsupervised domain adaptation. Office-31 contains 4,652 images in 31 categories, and consists of three domains: Amazon (A), Webcam (W), and DSLR (D). We evaluate the methods across the three domains, resulting in six transfer scenarios. Office-Home is a relative challenging dataset with 15,500 images in 65 categories. It has four significantly different domains: Artistic images (Ar), Clip Art (Cl), Product images (Pr), and Real-World images (Rw). There are 12 transfer tasks among four domains in total. 


\begin{table}[t]
	\begin{center}
		
		%\vspace{-12pt}
		
		\caption{Accuracies (\%) on Office-31 for ResNet50-based unsupervised domain adaptation methods.}
		\vspace{-10pt}
		\label{tableoffice}
		%\addtolength{\tabcolsep}{2pt}
			\setlength{\tabcolsep}{0.3mm}{ 
				\resizebox{0.48\textwidth}{!}{%
				\begin{tabular}{cccccccc}
					\hline
					Method & A$\rightarrow$D & A$\rightarrow$W & D$\rightarrow$W & W$\rightarrow$D & D$\rightarrow$A & W$\rightarrow$A & Avg \\
					\hline\hline
					ResNet-50 \cite{he2016deep} & 68.9 & 68.4 & 96.7 & 99.3 & 62.5 & 60.7 & 76.1 \\
					GFK \cite{gong2012geodesic} & 74.5 & 72.8 & 95.0 & 98.2 & 63.4 & 61.0 & 77.5 \\
					DAN \cite{long2015learning} & 78.6 & 80.5 & 97.1 & 99.6 & 63.6 & 62.8 & 80.4 \\
					DANN \cite{ganin2016domain} & 79.7 & 82.0 & 96.9 & 99.1 & 68.2 & 67.4 & 82.2 \\
					ADDA \cite{tzeng2017adversarial} & 77.8 & 86.2 & 96.2 & 98.4 & 69.5 & 68.9 & 82.9 \\
					MaxSquare \cite{chen2019domain}&90.0 &92.4 &\textbf{99.1} &\textbf{100.0}  &68.1 &64.2 &85.6\\
					Simnet \cite{pinheiro2018unsupervised} & 85.3 & 88.6 & 98.2 & 99.7 & {73.4} & 71.8 & 86.2 \\				
					GTA \cite{sankaranarayanan2018generate} & 87.7 & 89.5 & 97.9 & 99.8 & 72.8 & 71.4 & 86.5 \\
					MCD \cite{saito2018maximum} & {92.2} & {88.6} & {98.5} & \textbf{100.0} & {69.5} & {69.7} & {86.5} \\	
					CBST~\cite{zou2018unsupervised}  &86.5  &87.8  &98.5 &\textbf{100.0}  &70.9  &71.2  &85.8 \\
					CRST~\cite{zou2019confidence}   &88.7  &89.4  &98.9 &\textbf{100.0} &70.9  &72.6 &86.8\\				
					
					
					\hline
					EntMin  &86.0	&87.9	&98.4	&\textbf{100.0} 	&67.0		&63.7&83.8\\
					BFM &87.7	&86.9	&98.5	&\textbf{100.0}	&67.6	&63.0	&84.0 \\
					
					BNMax  & {90.3} & {91.5} & {98.5} & \textbf{100.0} & {70.9}  & {71.6} & {87.1} \\
					FBNMax &90.4 	&91.9 	&98.6 	&99.9 	&71.2 	&70.5 	&87.1\\ 
					BNM$^2$ &92.6 	&92.6 	&98.7 	&99.9 	&72.4 	&73.6 	&88.3 \\
					FBNM$^2$ &91.6 &92.7 &98.5 &100.0 	&72.1 &73.1 &88.0 \\				
					\hline
					CDAN \cite{long2018conditional} & {92.9} & \textbf{93.1} & {98.6} & \textbf{100.0} & {71.0} & {69.3} & {87.5} \\
					CDAN+EntMin &92.0	&91.2 &98.7	&\textbf{100.0}	&70.7		&71.0	&87.3\\
					CDAN+BNMax  & {92.9} & {92.8} & {98.8} & \textbf{100.0} & {73.5} & {73.8} & {88.6} \\
					CDAN+FBNMax & 92.7 	&92.4 		&98.6 &99.7 	&74.0 &73.7 		&88.5 \\
					CDAN+BNM$^2$ & {93.4} 		&92.7 		&99.0 &100.0 	&73.5 &75.5 	&{89.0}\\
					CDAN+FBNM$^2$ &92.6 		&92.4 			&99.0 &100.0 &{74.7} &{74.2} 	&{88.8} \\
					\hline
					SHOT~\cite{liang2020we}  &\textbf{94.0} &90.1  &98.4  &99.9 &74.7 &74.3&88.6 \\
					BNMax-S &93.0 	&93.0  &	98.2	&99.9  	&\textbf{75.4}	&74.9 	&\textbf{89.1} \\
					FBNMax-S &93.0 	&92.9  &98.2  &99.9 &\textbf{75.4}		&\textbf{75.0} &\textbf{89.1}\\
					\hline
			\end{tabular}}
			
		}
	\end{center}
	\vspace{-10pt}
\end{table}

\begin{table*}[htbp]
	\begin{center}
		\vspace{-5pt}
		
		\caption{Accuracies (\%) on Office-Home for ResNet50-based unsupervised domain adaptation methods.}
		%\vspace{-0.5pt}
		\label{tableofficehome}
		\addtolength{\tabcolsep}{-5.5pt}
		\scalebox{0.95}{
			\resizebox{\textwidth}{!}{%
				\begin{tabular}{cccccccccccccc}
					\hline
					Method& Ar$\rightarrow$Cl & Ar$\rightarrow$Pr & Ar$\rightarrow$Rw & Cl$\rightarrow$Ar & Cl$\rightarrow$Pr & Cl$\rightarrow$Rw & Pr$\rightarrow$Ar & Pr$\rightarrow$Cl & Pr$\rightarrow$Rw & Rw$\rightarrow$Ar & Rw$\rightarrow$Cl & Rw$\rightarrow$Pr & Avg \\
					\hline\hline
					
					ResNet-50 \cite{he2016deep} & 34.9 & 50.0 & 58.0 & 37.4 & 41.9 & 46.2 & 38.5 & 31.2 & 60.4 & 53.9 & 41.2 & 59.9 & 46.1 \\
					DAN \cite{long2015learning} & 43.6 & 57.0 & 67.9 & 45.8 & 56.5 & 60.4 & 44.0 & 43.6 & 67.7 & 63.1 & 51.5 & 74.3 & 56.3 \\
					DANN \cite{ganin2016domain} & 45.6 & 59.3 & 70.1 & 47.0 & 58.5 & 60.9 & 46.1 & 43.7 & 68.5 & 63.2 & 51.8 & 76.8 & 57.6 \\
					MCD \cite{saito2018maximum} &48.9	&68.3	&74.6	&61.3	&67.6	&68.8	&57	&47.1	&75.1	&69.1	&52.2	&79.6	&64.1 \\
					
					SAFN~\cite{Xu_2019_ICCV} &52.0&	71.7&76.3&64.2&69.9&71.9&63.7&51.4&	77.1&70.9&57.1&81.5&67.3\\
					Symnets \cite{zhang2019domain} & 47.7 & 72.9 & 78.5 & {64.2} & 71.3 & 74.2 & {64.2}  & 48.8 & 79.5 & {74.5} & 52.6 & {82.7} & 67.6 \\
					MDD \cite{zhang2019bridging} & 54.9 & 73.7 & 77.8 & 60.0 & 71.4 & 71.8 & 61.2 & 53.6 & 78.1 & 72.5 & \textbf{60.2} & 82.3 & 68.1 \\
					\hline
					
					EntMin  &43.2	&68.4	&78.4	&61.4	&69.9	&71.4	&58.5	&44.2	&78.2	&71.1	&47.6	&81.8	&64.5 \\
					BFM &43.3 	&69.1 	&78.0 	&61.3 	&67.4 	&70.9 	&57.8 	&44.1 	&78.9 	&72.1 	&50.1 	&81.0 	&64.5 \\
					BNMax &{52.3}	&{73.9}	&{80.0}	&63.3	&{72.9}	&{74.9}	&61.7	&{49.5}	&{79.7}	&70.5	&{53.6}	&82.2	&67.9\\	
					FBNMax &54.9 	&73.4 	&79.3 	&62.6 	&73.6 	&74.5 	&61.0 	&51.7 	&79.6 	&70.1 	&57.1 	&82.3 	&68.3\\
					BNM$^2$ &55.8 	&74.8 	&79.9 	&64.2 	&73.7 	&75.5 	&61.6 	&52.4 	&80.4 	&72.2 	&56.8 	&83.5 	&69.2\\ 
					FBNM$^2$ &55.3 	&75.4 	&79.9 	&64.0 	&74.2 	&75.5 	&62.2 	&52.0 	&80.4 	&72.3 	&57.0 	&83.4 	&69.3\\ 
					\hline
					CDAN \cite{long2018conditional} & 50.7 & 70.6 & 76.0 & 57.6 & 70.0 & 70.0 & 57.4 & 50.9 & 77.3 & 70.9 & 56.7 & {81.6} & 65.8 \\
					CDAN+EntMin &54.1	&72.4	&78.3	&61.8	&71.8	&73.0	&62.0	&52.3	&79.7	&72.0	&57.0	&83.2	&68.1 \\
					
					
					CDAN+BNMax &56.1 	&75.0 	&79.0 	&63.3 	&73.1 	&74.0 	&62.4 	&53.6 	&80.9 	&72.2 	&58.6 	&83.5 	&69.3 \\
					CDAN+BNM$^2$ &55.8 	&75.1 	&79.1 	&63.3 	&73.2 	&74.1 	&62.6 	&53.3 	&80.7 	&72.2 	&59.0 	&83.8 	&69.4\\
					CDAN+FBNMax &56.3 	&74.6 	&79.3 	&63.4 	&73.2 	&73.9 	&62.7 	&53.5 	&81.0 	&72.7 	&58.7 	&83.6 	&69.4\\
					CDAN+FBNM$^2$ &56.1 	&74.9 	&79.3 	&63.6 	&73.6 	&74.1 	&62.9 	&54.1 	&81.0 	&72.5 	&58.4 	&83.6 	&69.5\\
					\hline 
					HDAN~\cite{cui2020hda} &56.8 &75.2 &79.8 &65.1 &73.9 &75.2 &66.3 &56.7 &81.8 &\textbf{75.4} &{59.7} &\textbf{84.7} &70.9\\
					HDAN+BNMax &57.4 	&75.8 	&{80.3} 	&66.1 	&74.3 	&75.4 	&67.0 	&57.6 	&81.9 	&74.9 	&{59.7} 	&\textbf{84.7} 	&71.3 \\
					HDAN+BNM$^2$ &57.3 	&75.8 	&{80.3} 	&66.1 	&{74.7} 	&{75.8} 	&66.7 	&\textbf{58.0} 	&81.9 	&75.1 	&59.9 	&\textbf{84.7} 	&{71.4} \\
					HDAN+FBNMax &\textbf{57.6} 	&{75.9} 	&{80.3} 	&65.7 	&74.1 	&{75.8} 	&{66.8} 	&57.7 	&{82.0} 	&74.9 	&59.6 	&\textbf{84.7} 	&71.3 \\ 
					HDAN+FBNM$^2$ &57.4 	&75.7 	&80.2 	&{66.3} 	&74.5 	&75.7 	&67.5 	&57.9 	&81.9 	&75.2 	&{59.7} 	&\textbf{84.7} 	&{71.4} \\
					\hline
					SHOT~\cite{liang2020we} &57.1 &\textbf{78.1} &81.5 &68.0 &\textbf{78.2} &78.1 &67.4 &54.9 &82.2 &73.3 &58.8 &84.3 &71.8 \\
					
					FBNMax-S &56.9 	&77.7 	&81.6 	&\textbf{68.1} 	&77.6 	&79.2 	&\textbf{67.7} 	&55.3 	&\textbf{82.2} 	&73.7 	&59.8 	&\textbf{84.7} 	&{72.0} \\
					BNMax-S &{57.4} 	&77.8 	&\textbf{81.7} 	&67.8 	&77.6 	&\textbf{79.3} 	&67.6 	&55.7 	&82.2 	&73.5 	&59.5 	&\textbf{84.7} 	&\textbf{72.1}\\
					\hline
		\end{tabular}}}
		\vspace{-10pt}
	\end{center}
\end{table*}


We adopt ResNet-50 \cite{he2016deep} pre-trained on ImageNet \cite{deng2009imagenet} as our backbone. The batch size is fixed to be $36$ in our experiments, implemented with PyTorch~\cite{torch}. During the training of the network, we employ mini-batch stochastic gradient descent (SGD) with initial learning rate as 0.0001 and momentum of 0.9 to train our model. As a typical method, BNMax loss is directly combined with classification loss with the parameter $\lambda$ fixed to be $0.5$. When BNMax is combined with existing methods, the parameter $\lambda$ is fixed to be $0.25$. For each method, we run four random experiments and report the average accuracy, to obtain general performance. 




\begin{figure}[t]
	\begin{center}
		
		\begin{minipage}{.24\textwidth}
			\subfigure[Target]{
				\includegraphics[width=0.9\textwidth]{figure/1target.png}
				\label{entropytarget}}
		\end{minipage}
		\begin{minipage}{.24\textwidth}
			\subfigure[Source]{	
				\includegraphics[width=0.9\textwidth]{figure/1source.png}
				\label{entropysource}}
		\end{minipage}
	    \vspace{-3ex}
		\caption{Prediction discriminability for Ar $\rightarrow$ Cl. As a typical measurement, less entropy means more prediction discriminability. }
		\label{entropy}
	\end{center}
	\vspace{-3ex}
\end{figure}

\begin{figure}[t]
	\begin{center}
		\begin{minipage}{.22\textwidth}
			\subfigure[Ar $\rightarrow$ Cl]{	
				\includegraphics[width=0.9\textwidth]{figure/office2ArCl.jpg}
				\label{home1}}
		\end{minipage}
		\begin{minipage}{.22\textwidth}
			\subfigure[Ar $\rightarrow$ Pl]{
				\includegraphics[width=0.9\textwidth]{figure/office2ArPl.jpg}
				\label{home2}}
		\end{minipage}
		\vspace{-3ex}
		\caption{Diversity ratio on Office-Home for domain adaptation, calculated as the predicted diversity divided by the ground truth diversity. The predicted (ground truth) diversity is measured by the average number of predicted (ground truth) categories in randomly sampled batches.}
		%Diversity ratio on Office-Home for domain adaptation, calculated as the predicted diversity divided by the ground truth diversity. The predicted (ground truth) diversity is measured by the average number of predicted (ground truth) categories in randomly sampled batches.
		\label{diversity}
	\end{center}
	\vspace{-3ex}
\end{figure}

The results on Office-31 and Office-Home are shown in Table~\ref{tableoffice} and~\ref{tableofficehome}. On both Office-31 and Office-Home, as expected, BFM obtains similar results with EntMin, while BNMax achieves substantial improvement on average over other entropy-based methods. Surprisingly, BNMax obtains superior results compared with popular alignment-based comparison methods. The results show that Batch Nuclear-norm Maximization is effective for domain adaptation, especially on the difficult tasks where the baseline accuracy is relatively low, such as D$\rightarrow$A in Office-31 and Rw$\rightarrow$Cl in Office-Home. Beyond typical BNMax, we also construct framework of BNM$^2$, which achieves remarkable improvement, compared with BNMax. Meanwhile, the approximate method FBNMax achieves similar results with BNMax, FBNM$^2$ also achieves similar results compared with BNM$^2$. The results show that our approximation of nuclear-norm is suitable to replace original calculation of nuclear-norm in operations of both BNMax and BNMin.

\begin{table*}[t]
	\begin{center}
		\vspace{-5pt}
		\caption{ Accuracies (\%) on Balance Domainnet of ResNet50-based UDA methods.}
		
		\label{balancedomainnet}
		%\addtolength{\tabcolsep}{2pt}
		\vspace{-3mm}
		\resizebox{\textwidth}{!}{%
			\begin{threeparttable}
				\centering
				\setlength{\tabcolsep}{1.3mm}{
					\begin{tabular}{ccccccccccccccccc}% indicators prediction
						%\begin{tabular}{c|cccccccccccccc|cc}% indicators prediction
						\hline 
						
						\multirow{2}{*}{Methods} & \multicolumn{2}{c}{R$\rightarrow$C} & \multicolumn{2}{c}{R$\rightarrow$P} & \multicolumn{2}{c}{P$\rightarrow$C} & \multicolumn{2}{c}{C$\rightarrow$S} & \multicolumn{2}{c}{S$\rightarrow$P} & \multicolumn{2}{c}{R$\rightarrow$S} & \multicolumn{2}{c}{P$\rightarrow$R} & \multicolumn{2}{c}{Avg}\\
						
						&{Src} &{Tgt} &{Src} &{Tgt} &{Src} &{Tgt} &{Src} &{Tgt} &{Src} &{Tgt} &{Src} &{Tgt} &{Src} &{Tgt} &{Src} &{Tgt} \\
						
						\hline \hline
						
						\multicolumn{1}{c}{Baseline1 \cite{he2016deep}} &\textbf{84.1} 	&67.3 	&84.1 	&70.6 	&\textbf{73.1} 	&59.5 	&\textbf{77.5} 	&62.0 	&71.7 	&58.5 	&\textbf{84.1} 	&64.6 	&\textbf{73.1} 	&71.7 	&\textbf{78.3} 	&64.9 \\ %&\multicolumn{1}{c}{60.0}  
						
						\multicolumn{1}{c}{Baseline2 \cite{he2016deep}} &82.8 	&68.1 	&84.3 	&71.9 	&68.9 	&60.7 	&75.5 	&63.0 	&71.3 	&62.7 	&81.8 	&64.9 	&72.5 	&72.6 	&76.7 	&66.3 	  \\
						
						\multicolumn{1}{c}{DAN} &82.1 	&68.3 	&84.0 	&71.8 	&69.4 	&61.4 	&75.8 	&63.8 	&71.7 	&63.5 	&81.3 	&65.1 	&71.6 	&71.9 	&76.6 	&66.6  \\
						\multicolumn{1}{c}{DANN}&81.2 	&69.3 	&82.6 	&72.7 	&65.0 	&58.5 	&72.5 	&64.1 	&70.1 	&61.9 	&80.5 	&67.8 	&69.0 	&70.2 	&74.4 	&66.4 \\
						
						
						\multicolumn{1}{c}{ENT~\cite{grandvalet2005semi}} &82.0 &69.1 	&83.9 	&71.4 	&69.2 	&62.4 	&74.9 	&62.4 	&71.5 	&64.0 	&81.4 	&65.8 	&71.4 	&73.5 	&76.3 	&66.9  \\
						
						\multicolumn{1}{c}{SAFN~\cite{Xu_2019_ICCV}} &82.5 	&67.9 	&84.4 	&71.5 	&69.3 	&60.5 	&75.9 	&63.1 	&71.0 	&63.1 	&81.9 	&64.6 	&72.0 	&72.4 	&76.7 	&66.2  \\
						
						\multicolumn{1}{c}{CDAN~\cite{long2018conditional}} &80.8 	&70.2 	&82.1 	&73.0 	&66.9 	&61.8 	&72.9 	&65.8 	&70.0 	&63.2 	&80.2 	&69.3 	&69.7 	&71.1 	&74.7 	&67.8  \\
						\hline
						\multicolumn{1}{c}{BFM} &82.5 	&69.4 	&84.6 	&73.5 	&69.0 	&62.2 	&76.1 	&65.2 	&72.1 	&64.5 	&82.2 	&67.8 	&72.9 	&74.2 	&77.1 	&68.1\\
						\multicolumn{1}{c}{BNMax($K=1$)} &82.5 &	69.7 	&84.6 	&73.8 	&68.5 	&62.6 	&76.6 	&65.6 	&72.4 	&65.5 	&81.9 	&67.8 	&73.0 	&74.4 	&77.1 	&68.5  \\
						\multicolumn{1}{c}{BNMax($K=2$)} &82.4 	&70.2 	&84.4 	&74.2 	&69.2 	&63.8 	&76.0 	&65.9 	&72.2 	&65.7 	&81.4 	&67.9 	&73.1 	&74.6 	&77.0 	&68.9\\
						\multicolumn{1}{c}{BNMax($K=3$)} &82.4 	&70.5 	&84.4 	&74.2 	&69.3 	&63.4 	&75.9 	&65.8 	&72.2 	&65.6 	&81.3 	&68.1 	&73.1 	&74.7 	&77.0 	&68.9\\
						\multicolumn{1}{c}{BNM$^2$} &82.2 	&70.4 	&83.9 	&73.8 	&68.5 	&63.4 	&76.5 	&65.9 	&71.8 	&65.5 	&81.3 	&67.7 	&71.9 	&74.3 	&76.6 	&68.7  \\
						\multicolumn{1}{c}{FBNMax} &82.1 	&70.4 	&84.4 	&74.0 	&68.7 	&63.2 	&76.3 	&66.2 	&71.5 	&65.3 	&81.5 	&68.0 	&72.9 	&74.6 	&76.8 	&68.8  \\
						\multicolumn{1}{c}{FBNM$^2$} &82.1 &70.4 	&84.6 	&74.2 	&68.7 	&63.4 	&75.6 	&65.9 	&72.2 	&65.5 	&81.2 	&67.9 	&72.9 	&74.6 	&76.7 	&68.8  \\ 
						\hline
						\multicolumn{1}{c}{HDAN~\cite{cui2020hda}} &82.8 	&72.8 	&84.3 	&74.8 	&70.5 	&65.8 	&75.1 	&68.0 	&71.7 	&66.6 	&82.8 	&\textbf{71.6} 	&{73.0} 	&75.4 	&77.2 	&70.7  \\
						\multicolumn{1}{c}{HDAN+BNMax} &82.3 	&72.7 	&84.3 	&74.7 	&70.5 	&\textbf{66.1} 	&76.3 	&68.0 	&\textbf{72.6} 	&\textbf{67.7} 	&82.5 	&71.3 	&72.7 	&75.5 	&77.3 	&\textbf{70.9}  \\
						\multicolumn{1}{c}{HDAN+BNM$^2$} &82.2 	&72.9 	&84.2 	&75.2 	&69.4 	&65.1 	&75.3 	&67.7 	&71.7 	&66.8 	&82.0 	&71.2 	&72.5 	&75.1 	&76.8 	&70.6 \\ 
						\multicolumn{1}{c}{HDAN+FBNMax} &82.6 	&\textbf{73.2}	&\textbf{84.5} 	&\textbf{75.4} 	&69.4 	&65.1 	&76.0 	&\textbf{68.5} 	&72.0 	&67.0 	&82.3 	&\textbf{71.6} 	&72.7 	&\textbf{75.6} 	&77.1 	&\textbf{70.9} \\
						\multicolumn{1}{c}{HDAN+FBNM$^2$} &82.4 	&73.0 	&84.3 	&75.0 	&70.0 	&65.8 	&75.5 	&68.2 	&71.2 	&66.5 	&82.1 	&71.4 	&72.8 	&\textbf{75.6} 	&76.9 	&70.8\\
						%\multicolumn{1}{|c|}{Supervised} &-&-  &-&-   &-&-  &-&-  &-&-  &-&- &-&- &-&\multicolumn{1}{c|}{-} \\
						
						\hline
				\end{tabular}}
				\renewcommand{\labelitemi}{}
				\vspace{-5pt}
				%\begin{itemize}
				%\begin{tablenotes}
				%	\setlength{\itemsep}{0em}
				%	\setlength{\labelsep}{0em}
				%		\setlength{\topsep}{0em}
				%		\item %\hspace*{-0.25in} %\small{The applied backbone is Resnet34~\cite{he2016deep} and Avg means the average results on previous adaptation scenarios.}
				%	\end{itemize}
			\end{threeparttable}
		}
		%\vspace{-5pt}
	\end{center}
	\vspace{-10pt}
\end{table*}
\begin{figure*}
	\begin{center}
		\begin{minipage}{.98\textwidth}
			\begin{minipage}{.24\textwidth}
				\subfigure[Baseline]{	
					\includegraphics[width=0.9\textwidth]{figure/tsnebase.jpg}
					\label{tsne0}}
			\end{minipage}
			\begin{minipage}{.24\textwidth}
				\subfigure[BFM]{
					\includegraphics[width=0.9\textwidth]{figure/tsnebfm.jpg}
					\label{tsne1}}
			\end{minipage}
			\begin{minipage}{.24\textwidth}
				\subfigure[BNMax]{
					\includegraphics[width=0.95\textwidth]{figure/tsnebnm.jpg}
					\label{tsne2}}
			\end{minipage}
			\begin{minipage}{.24\textwidth}
				\subfigure[BNM$^2$]{
					\includegraphics[width=0.9\textwidth]{figure/tsnebnmm.jpg}
					\label{tsne3}}
			\end{minipage}
			
			
			
			%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
			%\includegraphics[width=.97\textwidth]{figure/tsne.png}
			
			\caption{T-SNE results of different methods on Ar $\rightarrow$ Cl.}
			\label{tsne}
		\end{minipage}
	\end{center}
	\vspace{-2ex}
\end{figure*}

Meanwhile, we add BNMax and BNM$^2$ to existing methods methods CDAN~\cite{long2018conditional} and HDAN~\cite{cui2020hda}, denoted as CDAN+BNMax, CDAN+BNM$^2$, HDAN+BNMax and HDAN+BNM$^2$ respectively. In terms of the performance, CDAN+BNMax outperforms CDAN and CDAN+EntMin by a large margin on both Office-31 and Office-Home. Besides, HDAN+BNMax performs better than HDAN on Office-Home, which also shows that BNMax could cooperate well with other methods. In terms of the improvement, BNMax is more suitable to improve CDAN and HDAN on the difficult tasks where the baseline accuracy is relatively low, such as D$\rightarrow$A and W$\rightarrow$A in Office-31, Ar$\rightarrow$Cl and Pr$\rightarrow$Cl in Office-Home. When cooperation with CDAN and HDAN, BNM$^2$ could still outperform BNMax on both Office-31 and Office-Home, which shows the necessity of BNMin. We also replace the methods of BNMax and BNM$^2$ by FBNMax and FBNM$^2$. The approximation methods of FBNMax and FBNM$^2$ achieve similar results compared with BNMax and BNM$^2$, which shows the effectiveness of the approximation. 

Recent work of SHOT~\cite{liang2020we} achieves well performed results, with similar constraint compared with BNMax. Thus we reproduce the results of BNMax under the same environment with SHOT. Since source data is not utilized in the training of SHOT, we could not apply BNM$^2$ to the framework. We replace the constraint on prediction diversity of information maximization by BNMax, and FBNMax, denoted as BNMax-S and FBNMax-S respectively.The reproduced results are shown in Table~\ref{tableoffice} and~\ref{tableofficehome}, which shows BNMax-S could also outperform SHOT on average on both Office-31 and Office-Home. Specifically, BNMax-S and FBNMax-S could achieve obvious improvement than SHOT on difficult tasks, such as D$\rightarrow$A in Office-31 and Rw$\rightarrow$Cl in Office-Home. The results show that simply limiting prediction discriminability and diversity by BNMax is enough for most cases. 


To analyze prediction discriminability for domain adaptation in BNMax, we calculate the typical measurement of entropy, as shown in Figure~\ref{entropy}. Compared with the baseline of source only, BNMax achieves less entropy and more prediction discriminability for target domain, as shown in Figure~\ref{entropytarget} during most of the training process. On source domain, as shown in Figure~\ref{entropysource}, BNM$^2$ could lessen prediction discriminability on source domain compared with BNMax. Though the differences seem to be little in the figure, the differences are still considerable, under the explicit constraint of cross entropy loss on source domain.

To validate that BNMax could maintain the diversity in domain adaptation, we show the diversity ratio in Office-Home on tasks of Ar $\rightarrow$ Cl and Ar $\rightarrow$ Pr in Figure~\ref{diversity}. Prediction diversity is measured by the average matrix rank, {i.e.}, mean number of predicted categories in randomly sampled batch. Thus the diversity ratio is measured by the average predicted category number dividing the average ground-truth category number. As shown in Figure~\ref{home1}, the diversity ratio of BNMax is larger than that of the EntMin by a large margin in Ar $\rightarrow$ Cl. The phenomenon is normal since the rich samples near the decision boundary are mainly classified into the majority categories, reducing the diversity in the batch examples. As shown in Figure~\ref{home2}, the diversity ratio of BNMax is still larger than that of the EntMin in Ar $\rightarrow$ Pl. But in Ar $\rightarrow$ Pl, the divergence between EntMin and BNMax in diversity ratio is less than the divergence in Ar $\rightarrow$ Cl. The lessened diversity differences result from fewer samples near the decision boundary in Ar $\rightarrow$ Pl. Less ambiguous samples in Ar $\rightarrow$ Pl could be explained by higher baseline accuracy in Ar $\rightarrow$. Thus BNMax is more effective in difficult tasks with rich data near the decision boundary. 

\begin{figure}[t]
	\begin{center}
		
		\begin{minipage}{.24\textwidth}
			\subfigure[Fixed Diversity]{
				\includegraphics[width=0.9\textwidth]{figure/rangediscri.png}
				\label{retio1}}
		\end{minipage}
		\begin{minipage}{.24\textwidth}
			\subfigure[Fixed Discriminability]{	
				\includegraphics[width=0.9\textwidth]{figure/rangediversity.png}
				\label{retio2}}
		\end{minipage}
		\vspace{-3ex}
		\caption{Accuracy under different radio between prediction discriminability and diversity. }
		\label{retio}
	\end{center}
	\vspace{-3ex}
\end{figure}

\begin{figure}[t]
	\begin{center}
		
		\begin{minipage}{.24\textwidth}
			\subfigure[Ar $\rightarrow$ Cl]{
				\includegraphics[width=0.9\textwidth]{figure/numArCl.png}
				\label{numArCl}}
		\end{minipage}
		\begin{minipage}{.24\textwidth}
			\subfigure[Ar $\rightarrow$ Pl]{	
				\includegraphics[width=0.9\textwidth]{figure/numArPl.png}
				\label{numArPl}}
		\end{minipage}
		\vspace{-3ex}
		\caption{Accuracy under different numbers of select categories under FBNM.}
		\label{numArClPl}
	\end{center}
	\vspace{-3ex}
\end{figure}
Towards the trade-off between improvement on prediction discriminability and diversity, we show the results with different ratios in Figure~\ref{retio}. Different ratios is achieved by harmonizing the results of $F$-norm and nuclear-norm. $F$-norm denotes the single discriminability while nuclear-norm denotes both discriminability and diversity. The weight of nuclear-norm is set to be $1$, when diversity is fixed. Under fixed diversity, both BNM and FBNM could reach optimal results when discriminability is set to be $1$, where the parameter of $F$-norm is set to be $0$. Meanwhile, the sum of weights for nuclear-norm and $F$-norm is fixed, when discriminability is fixed. Both BNM and FBNM reaches optimal solutions when diversity is set to be $1$. The results show that discriminability and diversity should be set with equal weights, which satisfies the circumstances of nuclear-norm.

To analyze the proper number of the selected categories for the fast method of FBNM. We show the accuracy under different numbers of select categories under FBNM in Figure~\ref{numArClPl}. The batch size is 36, and 36 categories are selected to approximate the nuclear-norm. While we find too large or too small number of selected categories will damage the overall accuracy. The results will reach optimal if the batch size is near 36. We also visualize the T-SNE results in Figure~\ref{tsne}, with source domain in blue and target domain in red. The visualization shows the large gap between source and target domain in Baseline, and the domain gap is reduced by increasing prediction discriminability in BFM. By integrating more categories, BNMax outperforms BFM in almost all the tasks. However, BNMax still suffers from the problem that the samples are not tightly connected. BNM$^2$ mitigate the problem by reducing the discriminability on source domain.




\begin{table}[t]
	\begin{center}
		%\vspace{-5pt}
		
		\caption{Partial comparisons on numbers of samples for categories.}
		\vspace{-8pt}
		\label{samplenum}
		%\addtolength{\tabcolsep}{-5.5pt}
		\setlength{\tabcolsep}{1.3mm}{
			%\resizebox{\textwidth}{!}{%
			\begin{tabular}{ccccccc}
				%\multicolumn{2}{c}{R$\rightarrow$C}
				\hline
				Dataset & Domain & Sum  & Mean & Std &Max &Min  \\
				\hline\hline
				\multirow{2}*{Office-31}  &Amazon &2817 	&90.9 	&13.5 	&100 	&36\\ 
				&Dslr &498 	&16.1 	&5.7 	&31 	&7 \\
				\hline
				\multirow{2}*{Office-Home}  &Art &2427 	&37.3 	&19.6 	&99 	&15	\\ 
				&Clipart &4365 	&67.2 &24.1 &99 &39	 \\
				\hline
				\multirow{4}*{Domainnet}  &Clipart (train) &34019&98.6 &55.3 &328 &8	\\ 
				&Clipart (test) &14814&42.9&	23.7 &141&4		 \\
				&Real (train)&122563	&355.3 	&121.0 	&570 &21 \\
				&Real (test) & 52764	&152.9 	&51.8 &245 &10	 \\
				\hline
				\multirow{4}*{\shortstack{Balance\\Domainnet}}  &Clipart (train) &6300&50 &0 &50 &50\\ 				
				&Clipart (test) &2772&22&	0 &22&22	 \\
				&Real (train)&8568	&68 	&0 	&68 &68 \\
				&Real (test) & 3780	&30 	&0 &30 &30	 \\
				\hline
		\end{tabular}}%}
		\vspace{-10pt}
	\end{center}
\end{table}

\subsection{Balance Domainnet}
To show the effect of our method, we also select balanced samples for the categories from Domainnet, called Balance Domainnet, selected from Domainnet~\cite{peng2019moment}. In Balance Domainnet, there are four domains including Real (R), Clipart (C), Painting (P) and Sketch (S) with larger domain discrepancy. Each domain holds total 126 categories, with at least 50 training samples for each category. To maintain balanced for the categories, different categories contain the same number of samples for one domain. The transfer tasks are selected by 7 domain adaptation scenarios, following the scenarios in \cite{saito2019semi}.

We also compare the number of samples in partial existing datasets as shown in Table~\ref{samplenum}, discussed in Supplementary in detail. We count the sum of samples (Sum), Mean category number (Mean), Standard category number (Std), Maximum category number (Max) and Minimum category number (Min). We could find that existing dataset of Office-31, Office-Home and Domainnet contains imbalanced categories, where the Std is always similar to Mean. Typically, In Clipart (train) of Domainnet, the largest sample number in categories is 328, while another category could only hold 8 samples. The imbalanced dataset would inevitably result in prediction bias, with improper conclusions in domain adaptation.


\begin{table}[t]
	\begin{center}
		\vspace{-5pt}
		
		\caption{Calculation time (s per 1000 times) under different $B$ and $C$.}
		\vspace{-8pt}
		\label{timetable}
		%\addtolength{\tabcolsep}{-5.5pt}
		\setlength{\tabcolsep}{1.3mm}{
			%\resizebox{\textwidth}{!}{%
			\begin{tabular}{ccccccc}
				\hline
				$B$ Number & $100$ & $100$ & $ 100$ & $1000$ & $10000$  & $1000$  \\
				$C$ Number & $100$ & $1000$ & $10000$ & $100$ & $100$  & $1000$  \\
				\hline
				
				BNMax	&0.89 	&2.72 	 &18.62	&1.93&6.39 &105.54	 	 \\
				EntMin~\cite{grandvalet2005semi}	&\textbf{0.05} 	&0.12 &1.80	&0.12 &1.64	&1.69 	 	 \\
				FBNMax &\textbf{0.05} 	&\textbf{0.11} 	&\textbf{0.82} &\textbf{0.08} &\textbf{0.30}  &\textbf{1.49}	 	\\
				
				\hline
				BNMax / FBNMax &16.34 	&23.88 &22.66 	&24.20 		&21.62 &70.78 	 \\ 
				\hline
		\end{tabular}}%}
		\vspace{-10pt}
	\end{center}
\end{table}


\begin{table*}[t]
	\begin{center}
		%\vspace{-5pt}
		\caption{ Accuracies (\%) on DomainNet subset of ResNet34-based SSDA methods.}
		
		\label{SSDA}
		%\addtolength{\tabcolsep}{2pt}
		\vspace{-5mm}
		\resizebox{\textwidth}{!}{%
			\begin{threeparttable}
				\centering
				\setlength{\tabcolsep}{0.3mm}{
					\begin{tabular}{ccccccccccccccccc}% indicators prediction
						%\begin{tabular}{c|cccccccccccccc|cc}% indicators prediction
						\hline 
						
						\multirow{2}{*}{Methods} & \multicolumn{2}{c}{R$\rightarrow$C} & \multicolumn{2}{c}{R$\rightarrow$P} & \multicolumn{2}{c}{P$\rightarrow$C} & \multicolumn{2}{c}{C$\rightarrow$S} & \multicolumn{2}{c}{S$\rightarrow$P} & \multicolumn{2}{c}{R$\rightarrow$S} & \multicolumn{2}{c}{P$\rightarrow$R} & \multicolumn{2}{c}{Avg}\\
						
						&{1$_{shot}$} &{3$_{shot}$} &{1$_{shot}$} &{3$_{shot}$} &{1$_{shot}$} &{3$_{shot}$} &{1$_{shot}$} &{3$_{shot}$} &{1$_{shot}$} &{3$_{shot}$} &{1$_{shot}$} &{\small{3-shot}} &{1$_{shot}$} &{3$_{shot}$} &{1$_{shot}$} &\multicolumn{1}{c}{3$_{shot}$} \\
						
						\hline \hline
						
						
						\multicolumn{1}{c}{ResNet34 \cite{he2016deep}} &55.6&60.0  &60.6&62.2   &56.8&59.4  &50.8&55.0  &56.0&59.5  &46.3&50.1 &71.8&73.9 &56.9&\multicolumn{1}{c}{60.0}  \\
						
						\multicolumn{1}{c}{DANN~\cite{ganin2016domain}} &58.2&59.8  &61.4&62.8   &56.3&59.6  &52.8&55.4  &57.4&59.9  &52.2&54.9 &70.3&72.2 &58.4&\multicolumn{1}{c}{60.7}  \\
						
						\multicolumn{1}{c}{ADR~\cite{saito2017adversarial}} &57.1&60.7  &61.3&61.9   &57.0&60.7  &51.0&54.4  &56.0&59.9  &49.0&51.1 &72.0&74.2 &57.6&\multicolumn{1}{c}{60.4} \\
						
						\multicolumn{1}{c}{CDAN~\cite{long2018conditional}} &65.0&69.0  &64.9&67.3   &63.7&68.4  &53.1&57.8  &63.4&65.3  &54.5&59.0 &73.2&78.5 &62.5&\multicolumn{1}{c}{66.5} \\
						
						\multicolumn{1}{c}{EntMin~\cite{grandvalet2005semi}} &65.2&71.0  &65.9&69.2   &65.4&71.1  &54.6&60.0  &59.7&62.1  &52.1&61.1 &75.0&78.6 &62.6&\multicolumn{1}{c}{67.6} \\
						
						\multicolumn{1}{c}{MME~\cite{saito2019semi}} &70.0&72.2  &67.7&69.7   &69.0&71.7  &56.3&61.8  &64.8&66.8  &61.0&61.9 &76.1&78.5 &66.4&\multicolumn{1}{c}{68.9} \\
						\multicolumn{1}{c}{GVBG~\cite{cui2020gvb}}&70.8	&	73.3&65.9&	68.7	&71.1 &	72.9	&62.4&	65.3 	&65.1 &		66.6	&67.1 &	68.5	&76.8	&79.2	&68.4	&	70.6\\
						
						%\multicolumn{1}{c}{CANN~\cite{opposite}} &\textbf{72.7}&\textbf{75.4}  &\textbf{70.3}&\textbf{71.5} &{69.8}&\textbf{73.2}  &{60.5}&{64.1} &\textbf{66.4}&\textbf{69.4}  &{62.7}&{64.2} &\textbf{77.3}&\textbf{80.8}  &{68.5}&\multicolumn{1}{c}{{71.2}} \\
						\hline
						\multicolumn{1}{c}{BNMax} &70.6 	&72.7 	&69.1 	&70.2 	&71.0 	&72.5 	&61.3 	&63.9 	&67.2 	&68.8 	&61.0 	&63.0 	&78.2 	&80.3 	&68.3 	&70.2 \\
						\multicolumn{1}{c}{BNM$^2$} &71.4 	&72.8 	&69.3 	&70.5 	&70.8 	&73.0 	&61.3 	&64.1 	&67.4 	&68.7 	&61.4 	&63.4 	&78.9 	&80.5 	&68.6 	&70.4 \\
						\multicolumn{1}{c}{FBNMax} &71.1 	&72.6 	&69.2 	&70.3 	&70.8 	&72.9 	&61.3 	&64.3 	&67.2 	&68.9 	&61.3 	&63.4 	&78.9 	&80.4 	&68.5 	&70.4 \\
						\multicolumn{1}{c}{FBNM$^2$} &71.0 &73.2 	&69.2 	&70.6 	&71.1 	&72.9 	&61.0 	&64.8 	&67.3 	&68.9 	&60.9 	&63.3 	&78.9 	&80.4 	&68.5 	&70.6 \\ 
						\hline
						\multicolumn{1}{c}{HDAN~\cite{cui2020hda}} &71.7 	&74.1 	&70.3 	&71.6 	&71.0 	&73.6 	&62.4 	&64.5 	&68.2 	&69.5 	&63.3 	&65.5 	&79.1 	&80.9 	&69.4 	&71.4 \\
						\multicolumn{1}{c}{HDAN+BNMax} &\textbf{72.5} 	&\textbf{74.5} 	&70.8 	&71.9 	&71.5 	&\textbf{74.3}	&\textbf{63.5} 	&64.7 	&68.8 	&70.1 	&63.8 	&\textbf{66.1} 	&\textbf{80.3} 	&\textbf{81.4} 	&\textbf{70.2}	&71.8 \\
						\multicolumn{1}{c}{HDAN+BNM$^2$} &* 	&74.5 	&\textbf{70.9} 	&\textbf{72.1} 	&71.7 	&\textbf{74.3}	&* 	&65.0 	&68.9 	&70.1 	&* 	&65.8 	&* 	&\textbf{81.4} 	&* 	&\textbf{71.9}\\ 	
						\multicolumn{1}{c}{HDAN+FBNMax} &71.8 &74.0 	&\textbf{70.9} 	&72.0 	&\textbf{72.0} 	&73.6 	&63.2 	&\textbf{66.5}	&69.0 	&\textbf{70.5} 	&\textbf{64.2} 	&65.8 	&79.8 	&81.2 	&70.1 	&\textbf{71.9}\\
						\multicolumn{1}{c}{HDAN+FBNM$^2$} &72.0 &73.6 	&70.8 	&72.0 	&71.9 	&73.7 	&63.3 	&66.3 	&\textbf{69.1} 	&70.4 	&\textbf{64.2} 	&65.9 	&79.8 	&81.3 	&\textbf{70.2} 	&\textbf{71.9}\\
						%\multicolumn{1}{|c|}{Supervised} &-&-  &-&-   &-&-  &-&-  &-&-  &-&- &-&- &-&\multicolumn{1}{c|}{-} \\
						
						\hline
				\end{tabular}}
				\renewcommand{\labelitemi}{}
				\vspace{-5pt}
				%\begin{itemize}
				%\begin{tablenotes}
				%	\setlength{\itemsep}{0em}
				%	\setlength{\labelsep}{0em}
				%		\setlength{\topsep}{0em}
				%		\item %\hspace*{-0.25in} %\small{The applied backbone is Resnet34~\cite{he2016deep} and Avg means the average results on previous adaptation scenarios.}
				%	\end{itemize}
			\end{threeparttable}
		}
		%\vspace{-5pt}
	\end{center}
	\vspace{-10pt}
\end{table*}


To explore our method under balanced circumstance, we show the results on Balance Domainnet in Table~\ref{balancedomainnet}. Baseline1 refers to model trained with source only, while Baseline2 refers to model trained with source only data along with updating the batch normalization (BN)~\cite{ioffe2015batch} layer with target unlabeled data. Updating BN layer could result in performance degradation on source domain, and increase the results on target domain. Directly increasing discriminability by BFM could achieve well-performed results on target domain. However, BNMax could still increase the results under balanced situations compared with BFM. The results validates that the prediction diversity is necessary even in a balanced dataset. Meanwhile, compared with Baseline2, BNMax could achieve higher performance on source domain, which also validates the effectiveness of BNMax.

Considering the large gap between batch size $B=36$ and category number $C=126$ in Balance Domainnet, we try different multiple number $K$, and we find BNMax could perform well when $K$ is $2$ or $3$. Thus BNMax could be fully explored when multiple $B$ is larger or a bit smaller than $C$. Meanwhile, BNMax could still improve the performance of HDAN. However, BNM$^2$ does not outperform BNMax under balanced dataset. The results show that the reduction of source domain does not provide improvement on performance, which means BNMin is more suitable for imbalanced small-scale source domain. The results also validate that balanced large-scale source domain hold less concern on overfitting, a conclusion easy to accept. In terms of the scenarios, BNMax could achieve well-performed results on difficult tasks, such as S$\rightarrow$P.
%The key insight of BNMin is to slightly reduce the performance on source domain, towards better transfer.


\begin{figure}[t]
	\begin{center}
		
		\begin{minipage}{.24\textwidth}
			\subfigure[Discriminability]{
				\includegraphics[width=0.9\textwidth]{figure/2discriRC.png}
				\label{balancediscriminability}}
		\end{minipage}
		\begin{minipage}{.24\textwidth}
			\subfigure[Diversity]{	
				\includegraphics[width=0.9\textwidth]{figure/2diversityRC.png}
				\label{balancediversity}}
		\end{minipage}
		\vspace{-3ex}
		\caption{Prediction discriminability and diversity for R$\rightarrow$C. Prediction discriminability is shown by entropy, while diversity is measured by average matrix rank dividing the average ground-truth category number. }
		\label{balanceentropy}
	\end{center}
	\vspace{-3ex}
\end{figure}

Under balanced situation, the prediction discriminability and diversity are shown in Figure~\ref{balanceentropy}. BNMax and EntMin could both increase prediction discriminability as shown in Figure~\ref{balancediscriminability}. Since EntMin is focused on only discriminability, more discriminability could be achieved in EntMin. On the other hand, though with slight advantages, BNMax could still increase the prediction diversity compared with EntMin as shown in Figure~\ref{balancediversity}. In Table~\ref{balancedomainnet}, BNMax could achieve more accurate predictions compared with EntMin. The comparison shows that prediction discriminability and diversity should both be increased, even in balanced situation.

To show that the approximation could speed up the training procedure, we calculate typical measurements in Table~\ref{timetable}. The results are shown in Pytorch on devices of CPU Intel(R) Core(TM) i7-4790K CPU @ 4.00GHz with 4 cpu cores. We run the results by randomly generate matrix $A$, to calculate typical measurements, and the time generating matrix $A$ is removed from the calculation time. We calculate the total time of measurements on $1000$ random matrix $A$. We denote the training time of BNMax dividing FBNMax as BNMax/FBNMax. The results show that FBNMax is faster than EntMin and BNMax for all the situations. As an approximation method, FBNMax could greatly shorten the calculation time of BNMax, such as $105.54$ to $1.49$ in matrix with $B=1000$ and $C=1000$. Also, we could find the gradual improvement on BNMax/FBNMax, from $B=100$ and $C=100$ to $B=1000$ and $C=1000$. The results show that FBNMax could reduce the computation complexity by approximately $n$, which also validate that FBNMax reduce  the computation complexity from $O(n^3)$ to $O(n^2)$.

\subsection{Semi-supervised Domain Adaptation}
% in domain adaptation
Semi-supervised domain adaptation (SSDA) is a more realistic setting, where domain adaptation is performed with labeled source data to partially labeled target data. In SSDA, we utilize typical dataset of semi Domainnet proposed in~\cite{saito2019semi}, which is selected from DomainNet~\cite{peng2019moment}. We take the same protocol with~\cite{saito2019semi} where the four domains including Real (R), Clipart (C), Painting (P) and Sketch (S) in total 126 categories. In this paper, following \cite{saito2019semi}, seven domain adaptation scenarios are formulated on the four domains, showing different levels of domain gap. All the methods are evaluated under the one-shot and three-shot settings the same with~\cite{saito2019semi}, where there are only $1$ or $3$ labeled samples per category in target domain.

We use ResNet34~\cite{he2016deep} as the backbones of the generator, optimized by SGD. The initial learning rate is $0.001$, with the momentum of $0.9$. BNMax loss is combined with classification loss with the parameter $\lambda$ fixed to $0.5$. When BNMax is regarded as a typical method, the source batch size is $24$ and target batch size is $48$, with multiple number as $1$. When BNMax is combined with existing methods, the source and target batch size is $24$, with the multiple number as $3$. Towards general performance for each method, we run three random experiments and report the average accuracy. 
%the parameter $\lambda$ is fixed to $1$, with

The quantitative results on semi DomainNet are summarized in Table~\ref{SSDA}. It is easily observed that BNMax outperforms comparisons on most settings, and achieves well performed results on average. The simple BNMax method outperforms adversarial training on entropy minimization by a large margin, especially in difficult scenarios such as $1_{shot}$ and $3_{shot}$ C$\rightarrow$S. Meanwhile, to show the effect of BNMax under SSDA, we also combine BNMax with existing method of HDAN. The improvement on HDAN means that existing method might still lack of enough prediction discriminability and diversity. 

Compared with the basic BNMax, BNM$^2$ could further improve the performance on both $1$ shot and $3$ shot situations. Surprisingly, FBNMax achieves better results compared with BNMax, which shows the superiority of the approximate method. When cooperated with HDAN, BNM$^2$ could still slightly outperform BNMax in most cases. However, in some scenarios, the training process might not converge, denoted as $*$ on performance, such as $1_{shot}$ R$\rightarrow$C. The converge problem results from the complex computation of singular value decomposition, and the iteration in the decomposition process. Compared with original calculation of nuclear-norm, our approximate method could figure the problem of the convergence by simply combining the components.
%HDAN also achieves significant improvement on one-shot SSDA, which shows the superiority of HDAN. 
% For example, compared with CANN, our method improves significantly on the difficult tasks, such as ${R} \rightarrow {S}$.

\subsection{Unsupervised Open Domain Recognition}
\label{exp}


For unsupervised open domain recognition, we evaluate our methods on I2AwA~\cite{zhuo2019unsupervised}. In I2AwA, source domain consists of 2,970 images belonging to 40 known categories, via selecting images from ImageNet and Google image search engine. Target domain of I2AwA is AwA2~\cite{aw2} which contains 37,322 images in total. The target images belong to 50 categories, the same 40 known categories with source domain, and the remaining 10 individual classes as unknown categories. 

To obtain reliable initial task model on unknown categories, we construct the same knowledge graph for I2AwA with UODTN~\cite{zhuo2019unsupervised}. The graph structure is constructed according to Graph Convolutional Networks (GCN) \cite{kipf2016semi,zgcn}. The graph nodes include all categories of target domain and the children and ancestors of the categories in WordNet~\cite{wordnet}. To obtain features of the nodes, we utilize the word vectors extracted via the GloVe text model~\cite{GloVe} trained on Wikipedia. We use ResNet50~\cite{he2016deep} pretrained on ImageNet~\cite{deng2009imagenet} as our backbone. The parameters of the last fully connected layer are initialized by the parameters of GCN in the same categories.  

\begin{table}
	\caption{Accuracies (\%) and other measurements on I2AwA for ResNet50-based unsupervised open domain recognition methods.}
	%\vspace{-2ex}
	\begin{center}
		\label{I2AwA}
		\vspace{-3pt}
		\setlength{\tabcolsep}{0.5mm}{
			\begin{tabular}{cccccccc}
				\hline               Method  &Discri.   &Diversity &Time  &Known        &Unknown         &All      &Avg     \\
				\hline\hline
				zGCN~\cite{zgcn}  &.&.   &.&77.2         &21.0            &65.0    &49.1    \\
				dGCN~\cite{adgpm}    &.&.  &.       &78.2        &11.6            &64    &44.9    \\
				adGCN~\cite{adgpm}    &.&.  &.      &77.3         &15.0           &64.1   &  46.2   \\
				bGCN~\cite{ubias}      &.&. &.      &84.6         &28.0           &72.6     &56.3  \\	
				pmdbGCN~\cite{pmd}     &.&.  &.    &84.7         &27.1           &72.5    &55.9  \\	
				UODTN~\cite{zhuo2019unsupervised}       &.&.  &.        &84.7 &31.7   &73.5&58.2\\
				
				Balance*~\cite{zhuo2019unsupervised}  &-0.759 &0.945 &1665.0		&85.9 &22.3	&72.4 &54.1\\	
				
				\hline
				EntMin &\textbf{-0.216} &0.839 &1786.3 &87.5&7.2	&70.5	&47.4\\
				BFM	&-0.260
				& 0.852 &1678.3&87.7 &9.2	&71.1	&48.4 \\				
				
				BNMax        & -0.246 &0.951   & 1768.3 &\textbf{88.3} &{39.7}   &{78.0}&{64.0}\\
				BNM$^2$ &-0.398 &0.950 & 1779.4 &85.2 	&\textbf{49.5} &77.6	&{67.4} \\
				
				FBNMax &-0.314 &\textbf{0.969}&\textbf{1661.9} &88.0 &43.6 &78.6  &65.8 \\
				FBNM$^2$ &-0.329 &0.962 &1663.0 &87.4 &49.2 &\textbf{79.3} &\textbf{68.3} \\
				
				
				\hline
			\end{tabular}
		}
	\end{center}
	\label{I2AwA}
	\vspace{-3ex}
\end{table}

\begin{figure*}
	\begin{center}
		\begin{minipage}{.98\textwidth}
			\begin{minipage}{.24\textwidth}
				\subfigure[All Category Accuracy]{	
					\includegraphics[width=0.9\textwidth]{figure/4acc.jpg}
					\label{compare1}}
			\end{minipage}
			\begin{minipage}{.24\textwidth}
				\subfigure[Known Category Accuracy]{
					\includegraphics[width=0.9\textwidth]{figure/4knownacc.jpg}
					\label{compare0}}
			\end{minipage}
			\begin{minipage}{.24\textwidth}
				\subfigure[Unknown Category Accuracy]{
					\includegraphics[width=0.95\textwidth]{figure/4preacc.jpg}
					\label{compare3}}
			\end{minipage}
			\begin{minipage}{.24\textwidth}
				\subfigure[Unknown Category Ratio]{
					\includegraphics[width=0.9\textwidth]{figure/4percent.jpg}
					\label{compare2}}
			\end{minipage}
			
			
			
			%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
			%\includegraphics[width=.97\textwidth]{figure/tsne.png}
			
			\caption{Statistics for Entropy, Balance and Nuclear-norm in the whole training process for unsupervised open domain recognition.}
			\label{compare}
		\end{minipage}
	\end{center}
	\vspace{-2ex}
\end{figure*}


For fair comparison, we perform in the same environment with UODTN~\cite{zhuo2019unsupervised}. The experiments are implemented by Pytorch~\cite{torch}. We fix the batch size to $48$ for both source and target domain. We apply BNMax on the classfication outputs on the total 50 categories and minimize classification loss on the known 40 categories in source domain and BNMax loss on all the 50 categories for target domain to train the network. Parameter $\lambda$ is set to be $2$ for BNMax, FBNMax and FBNM$^2$, while $1$ for BNM$^2$. We report the prediction results of known categories, unknown categories, all target categories, the average of known and unknown category accuracy, along with the measurements of prediction discriminability and diversity. The prediction discriminability (denoted as Discri. in short) is measured by negative entropy to ensure more discriminability with more negative entropy. While prediction diversity is measured by average predicted matrix rank dividing average ground truth matrix rank. To show the superiority of approximation, we also calculate the training time for 6000 iterations on device of GeForce RTX 3090, denoted as Time. For each method, we run four random experiments and report the average result. 

\begin{table}
	\caption{Parameter Sensitivity on the I2AwA dataset for ResNet50-based unsupervised open domain recognition methods.}
	%\vspace{-2ex}
	\begin{center}
		\label{I2AwA}
		%\vspace{-1pt}
		\setlength{\tabcolsep}{0.5mm}{
			\begin{tabular}{cccccccc}
				\hline                Method    &Discri.   &Diversity &Time  &Known        &Unknown         &All      &Avg    \\
				\hline	\hline
				BNMax ($\lambda=1$) &0.340 &0.952 &1768.4	         &{88.0}&{39.4}   &{77.7}&{63.7}\\
				BNMax ($\lambda=1.5$) &0.290 &0.956 &1770.2 
				&{88.1}&\textbf{39.7}   &{77.9}&{63.9}\\
				BNMax ($\lambda=2$)  &0.246 &0.951 &1768.3 &\textbf{88.3}&\textbf{39.7}   &\textbf{78.0}&\textbf{64.0}\\
				BNMax ($\lambda=3$) &0.208 &0.958 &1772.8 &{87.7} &{39.5}   &{77.5}&{63.6}\\
				BNMax ($\lambda=4$) &\textbf{0.183} &\textbf{0.962} &\textbf{1767.4} &{87.4} &{38.6}   &{77.1}&{63.0}\\
				\hline
			\end{tabular}
		}
	\end{center}
	\label{stable}
	\vspace{-3ex}
\end{table}
%TODO bGCN
The results are shown in Table~\ref{I2AwA}, we achieve remarkable improvement on I2AwA. Ffom the view of prediction accuracy, we achieve 11.4\% improvement on the known categories compared with the baseline zGCN, and BNMax surprisingly improves by 19.0\% on the unknown categories over zGCN. From the overall range of the dataset, we achieve 13.3\% improvement on the whole dataset and we achieve an average improvement of 15.2\% improvement over zGCN. Besides, BNMax outperforms the state-of-the-art UODTN~\cite{zhuo2019unsupervised} by 4.8\%. The results show that the simple BNMax is effective enough for unsupervised open domain recognition, which outperforms the combination of complex functions in UODTN. Besides, compared with BNMax, BNM$^2$ could achieve higher average of known and unknown category accuracy by promoting more accurate predictions on unknown categories. Surprisingly, the approximated methods of FBNMax and FBNM$^2$ could achieve more accurate predictions both on all sample accuracy and average category predictions, compared with BNMax and BNM$^2$. Among our methods, FBNM$^2$ achieves best results on both accuracy of All and Avg, with 10.1\% improvement on Avg and 5.8\% improvement on All compared with UODTN. 

Also, BNMax could improve typical measurements of discriminability and diversity. Compared with Balance, BNMax could improve the prediction discriminability from $-0.759$ to $-0.246$. Though EntMin could ensure more prediction discriminability, excessively increasing discriminability seems to be unsatisfying. In terms of prediction diversity, the diversity ratio is improved from $0.839$ to $0.969$ from EntMin to BNMax. We also find that the approximation method could achieve better prediction results by ensuring more prediction diversity. From BNMax to FBNMax, diversity ratio changes from $0.951$ to $0.969$, with all accuracy from $78.0$ to $78.6$ and average accuracy from $64.0$ to $65.8$. In terms of the training time, the approximated methods hold the advantages of the training time, with reduction from $1768.3$ to $1661.9$ second by replacing BNMax to FBNMax.

We show the parameter sensitivity experiments in Table~\ref{stable}. The results show BNMax is relatively stable under different $\lambda$, such as the training time, known category accuracy and all samples accuracy. In terms of $\lambda$, the performance of All and Avg reaches the highest when $\lambda$ equals $2$. As for the transfer properties, larger $\lambda$ means relatively more prediction discriminability and diversity for target domain. Too higher prediction discriminability and diversity could reduce the knowledge learned by source domain. Thus proper value of $\lambda$ is also important for the methods, and we set $\lambda$ fixed to $2$ for further comparison.

We also compare the training process of EntMin, Balance and BNMax loss functions in Figure~\ref{compare}. The prediction results on all categories, known categories and unknown categories are separately shown in Figure~\ref{compare1},~\ref{compare0} and~\ref{compare3}. BNMax outperforms comparisons on all accuracy, known category accuracy and unknown category accuracy in the whole training process. To explore the intrinsic effect of BNMax on unknown categories, we show the unknown category ratio, which is the ratio of predicting the samples in target domain of I2AwA into unknown categories in Figure~\ref{compare2}. Obviously, EntMin reduces the unknown category ratio by a large margin, which greatly damages the prediction diversity and accuracy on unknown categories. Though the unknown category ratio in BNMax is reduced at first, it gradually raises along the training process, and it appears to be even higher than initial ratio after training. This means BNMax could increase prediction diversity by ensuring ratio of predictions on minority categories. Though the Balance constraint could also protect ratio of prediction on minority categories, results of Balance loss seems not quite stable. Besides, the accuracy of Balance loss is much lower than BNMax due to the lack of discriminability. The experimental phenomenon has steadily proved the effectiveness of BNMax towards both discriminability and diversity.

\subsection{Discussion}

The chosen tasks are typical domain adaptation circumstances to show the effect of BNMax. Among the tasks and datasets, there are mainly differences in three aspects, {\it i.e.}, the domain discrepancy, category imbalance ratio and category number. There exists less domain discrepancy for Office-31, while large domain discrepancy for other datasets. From the balance view, the categories are only balanced in Balance Domainnet of UDA. While in Office-31 and Office-Home of UDA and semi-Domainnet of SSDA, the categories are imbalanced. Meanwhile, I2AwA of UODR is a task with extremely imbalanced category distributions, where some categories are even unseen in source domain. In terms of the category number, the category number is relative small in Office-31, Office-Home and I2AWA, while relative large in semi Domainnet and Balance Domainnet.

In terms of domain discrepancy, BNMax could perform well in most cases. Thus BNMax is suitable for both large and small domain discrepancy, while experiments show that BNMax could obviously improve the results when large domain discrepancy exists. In terms of the imbalance ratio, BNMax could perform on strictly balanced dataset of Balance Domainnet, and also other imbalanced domain adaptation scenarios. Therefore, in both imbalanced and balanced situations, maintaining prediction diversity by BNMax is necessary. In UODR, the simple structure of BNMax could even achieve state-of-the-art results, thus BNMax could perform better under imbalanced situations. 

Among the tasks, BNM$^2$ outperforms BNMax in most cases, except Balance Domainnet. Since the differences between BNM$^2$ and BNMax lie in BNMin, BNMin should perform under imbalanced small-scale circumstance. In BNMax, batch size should not be too small compared with category number. In Office-31, Office-Home and I2AWA the category number is similar to the batch size, and BNMax performs well. While in Balance Domainnet and semi Domainnet, we are required to enlarge the batch size towards better performance. 

%As shown in the experiments, BNMax could cooperate well with existing methods in semi-supervised learning. For domain adaptation, BNMax could outperform most existing methods using losses such as adversarial loss. While in unsupervised open domain recognition, method with only the BNMax loss and classification loss could even achieve state-of-the-art results. We could see the progressive progress and fitness of BNMax to the tasks, from semi-supervised learning to unsupervised open domain recognition. Considering the differences between the tasks, we could obtain two conclusions on the applicability of BNMax. The first is that BNMax could work well in label insufficient situations. The other is that BNMax outperforms entropy minimization significantly, especially when there exists rich domain discrepancy and imbalanced category distribution. 






